Probing eV-mass scale axions with a Micromegas detector in the CAST experiment

The CAST (CERN Axion Solar Telescope) experiment is searching for axions, an hypothetical particle that emerges as a possible solution to the well known CP violation problem in strong interactions. CAST is using a decommissioned LHC dipole magnet able to track the Sun as a possible source of solar axions, and to convert them to X-rays photons detectable with low background X-ray detectors. CAST continues its data taking period scanning masses up to 1eV. This thesis presents the data obtained with a Micromegas detector for the scanned axion mass range up to 0.64eV. The working principle, characterization and analysis of the Micromegas detectors operating in CAST are detailed in this work. Moreover, the last detector data corresponding to the new data taking period, with 3He gas inside the bores, was used to obtain a preliminar and conservative upper limit on the axion-photon coupling for the new axion mass range explored, g_{a\gamma} < 2.44 10^{-10} GeV^{-1}.

==> bibliography.tex <==
%\addcontentsline{toc}{chapter}{Bibliography}
\bibliographystyle{unsrt}
\begin{thebibliography}{100}
\bibitem{Dafni:2009df}
  T. Dafni {\it et al.},
  Energy resolution of alpha particles in a Micromegas detector at high pressure,
  {\it Nucl. Instrum. Meth. A} {\bf 608} (2009) 259.

\bibitem{Dafni:2008df}
  T. Dafni {\it et al.},
  New Micromegas detectors for rare event searches: axions and $\beta\beta$ decay,
  {\it Preprint}: PoS(idm 2008)106.
  Proceedings of the 7th International Workshop on The Identification of Dark Matter.

\bibitem{Dafni:2008df2}
  T. Dafni {\it et al.},
  MICROMEGAS for Rare Event Searches,
  Proceedings of the IEEE 2008, Dresden.

\bibitem{Iguaz:2008fi}
  F. J. Iguaz {\it et al.},
  Energy resolution of alpha particles in a Micromegas detector at high pressure,
  Proceedings of the 4th Symposium on Large TPCs for Low Energy Rare event Detection,
  {\it J. Phys. Conf. Ser.} {\bf 179} (2009) 012007.

\bibitem{Tomas:2009at}
  A. Tom\'as {\it et al.},
  Development of Micromegas towards Double Beta Neutrinoless Decay Searches,
  {\it JINST} {\bf 4} (2009), P11016,
  Proceedings of the 1st International Conference on Micro Pattern Gaseous Detectors (MPGD2009), Crete.

\bibitem{Reines:1959fr}
  F. Reines and C.~L. Cowan,
  Free Antineutrino Absorption Cross Section. I. Measurement of the Free Antineutrino Absorption Cross Section by Protons,
  {\it Phys. Rev.} {\bf 113} (1959) 273.

\bibitem{Fatemi-Ghomi:2009nfg}
  N. Fatemi-Ghomi,
  Measurement of the Double Beta Decay Half-life of $^{150}$Nd and Search for Neutrinoless Decay Modes with the NEMO3 Detector,
  PhD Thesis, University of Manchester, 2009.

\bibitem{Elliot:2002se}
  S.~R. Elliot and J. Engel,
  Double Beta Decay,
  {\it Preprint} arXiv:hep-ph/0202264.

\bibitem{Simkovi:2009fs}
  F. Simkovic {\it et al},
  The $0\nu\beta\beta$-decay nuclear matrix elements with self-consistent short range correlations,
  {\it Phys. Rev. C} {\bf 79} (2009) 055501,
  {\it Preprint} arXiv:nucl-th/09020331.

\bibitem{Menendez:2008jm}
  J. Men\'endez and A. Poves,
  Disassembling the Nuclear Matrix Elements of the Neutrinoless $\beta\beta$ Decay,
  {\it Nucl. Phys. A} {\bf 818} (2009) 139,
  {\it Preprint} arXiv:nucl-th/08013760.

\bibitem{KK:2001kk}
  H. Klapdor-Kleingrothaus {\it et al.},
  First Evidence for Lepton Number Violation and of the Majorana Character of Neutrinos,
  {\it Modern Physics Letters A}  {\bf 16} (2001) 2409.

\bibitem{Aalseth:2002cea}
  C.~E. Aalseth {\it et al.},
  IGEX $^{76}$Ge neutrinoless double-beta decay experiment: Prospects for next generation experiments,
  {\it Phys. Rev. D} {\bf 65} (2002) 092007.

\bibitem{Luescher:1998rl}
  R. Luescher {\it et al.},
  Search for $\beta\beta$ decay in $^{136}$Xe: new results from the Gotthard experiment,
  {\it Phys. Lett. B} {\bf 434} (1998) 407.

\bibitem{Giomataris:1996yg}
  Y. Giomataris, P. Rebourgeard, J.~P. Robert and G. Charpak,
  MICROMEGAS: A high - granularity position - sensitive gaseous detector for high particle - flux environments,
  {\it Nucl. Instrum. Meth. A} {\bf 376} (1996) 29.

\bibitem{Colas:2004pc}
  P. Colas, I. Giomataris and V. Lepeltier,
  Ion backflow in the Micromegas TPC for the future linear collider,
  {\it Nucl. Instrum. Meth. A} {\bf 535} (2004) 226.

\bibitem{Papaevangelou:2009tp}
  T. Papaevangelou {\it et al.},
  Development and performance of Microbulk Micromegas detectors,
  Proceedings of the 1st International Conference on Micro-Pattern Gaseous Detectors (MPDG 2009), to be published.

\bibitem{Dolbeau:2005kt}
  J. Dolbeau, I. Giomataris, P. Gorodetzky, T. Patzak, P. Salin and A. Sarat,
  The solar neutrino HELLAZ project,
  {\it Nucl. Phys. Proc. Suppl.} {\bf 138} (2005) 94.

\bibitem{Hanlon:2003joh}
  J.~F. O'Hanlon,
  A User's Guide to Vacuum Technology,
  3rd Edition (2003), John Wiley and Sons, Inc.

\bibitem{Ackerman:2009na}
  N. Ackerman {\it et al},
  Status of EXO-200,
  Proceedings of the DPF-2009 Conference, Detroit, MI, July 27-31, 2009 1.

\bibitem{Bernabei:2003rb}
  R. Bernabei {\it et al.},
  Investigation of $\beta\beta$ decay modes in $^{134}$Xe and $^{136}$Xe,
  {\it Phys. Lett. B} {\bf 546} (2002) 23.

\bibitem{Ball:2009mb}
  M. Ball {\it et al.}
  NEXT: A Neutrinoless Double Beta Decay Experiment,
  IEEE Transactions On Nuclear Science 2009.

\bibitem{Castell:2010jc}
  J. Castell,
  design reproduced with permission.

\bibitem{Morales:1999am}
  A. Morales,
  Review on Double Beta Decay Experiments $\&$ Comparison with Theory,
  {\it Nucl. Phys. (Proc. Suppl.)} {\bf 77} (1999), 335-345.

\bibitem{Elliot:2004se}
  S.~R. Elliot and J. Engel,
  Double Beta Decay,
  {\it J. Phys G} {\bf 30} (2004), R183.

\bibitem{Avignone:2005cs}
  F.~T. Avignone, G.~S. King and Yu.~G. Zdesenko,
  Next generation double beta decay experiments: Metrics for their evaluation,
  {\it New J. Phys.} {\bf 7} (2005) 6.

\bibitem{Caldwell:2001dc}
  D.~O. Caldwell (Editor),
  Current Aspects of Neutrino Physics,
  Springer, Berlin, 2001.

\bibitem{Goeppert:1935mg}
  M. Goeppert-Mayer,
  Double Beta-Disintegration,
  {\it Phys. Rev.} {\bf 48} (1935) 512.

\bibitem{Majorana:1937em}
  E. Majorana,
  Teor\'ia simmetrica dell'electrone e del positrone,
  {\it Nuovo Cimento} {\bf 14} (1937) 171.

\bibitem{Reines:1965fr}
  F. Reines {\it et al.},
  Evidence for High-Energy Cosmic-Ray Neutrino Interactions,
  {\it Phys. Rev. Lett.} {\bf 15} (1965) 429.

\bibitem{Davis:1968rd}
  R. Davis, D.~S. Harmer and K.~C. Hoffman,
  Search for Neutrinos from the Sun,
  {\it Phys. Rev. Lett.} {\bf 20} (1968) 1205.

\bibitem{Danby:1962gd}
  G. Danby {\it et al.},
  Observation of High-Energy Neutrino Reactions and the Existence of Two Kinds of Neutrinos,
  {\it Phys. Rev. Lett.} {\bf 9} (1962) 36.

\bibitem{Abrams:1989gsa}
  G.~S. Abrams {\it et al.},
  Measurements of Z-boson resonance parameters in e$^+$e$^-$ annihilation,
  {\it Phys. Rev. Lett.} {\bf 63} (1989) 2173.

\bibitem{Decamp:1990dd}
  D. Decamp {\it et al.},
  A precise determination of the number of families with light neutrinos and of the Z boson partial widths,
  {\it Phys. Lett. B} {\bf 235} (1990) 399.

\bibitem{Kodama:2001kk}
  K. Kodama {\it et al.},
  Observation of tau neutrino interactions,
  {\it Phys. Lett. B} {\bf 504} (2001) 218.

\bibitem{Hirata:1989kh}
  K.~S. Hirata {\it et al.},
  Observation of 8B solar neutrinos in the Kamiokande-II detector,
  {\it Phys. Rev. Lett.} {\bf 63} (1989) 16.

\bibitem{Pontecorvo:1958bp}
  B. Pontecorvo,
  Mesonium and Antimesonium,
  {\it J. Exptl. Theoret. Phys.} {\bf 33} (1957) 549.

\bibitem{Maki:1962mns}
  Z. Maki, M. Nakagawa, and S. Sakata,
  Remarks on the unified model of elementary particles,
  {\it Prog. Theor. Phys.} {\bf 28} (1962) 870.

\bibitem{Beckker-Szendy:1992rbs}
  R. Becker-Szendy {\it et al.},
  Electron- and muon-neutrino content of the atmospheric flux
  {\it Phys. Rev. D.} {\bf 46} (1992) 3720.

\bibitem{Fukuda:1994yf}
  Y. Fukuda {\it et al.},
  Atmospheric $\nu_\mu$/$\nu_e$ ratio in the multi-GeV energy range,
  {\it Phys. Lett. B} {\bf 335} (1994) 237.

\bibitem{Fukuda:1998yf}
  Y. Fukuda {\it et al.},
  Evidence for Oscillation of Atmospheric Neutrinos,
  {\it Phys. Rev. Lett.} {\bf 81} (1998) 1562.

\bibitem{Eguchi:2003ke}
  K. Eguchi {\it et al.},
  First Results from KamLAND: Evidence for Reactor Antineutrino Disappearance,
  {\it Phys. Rev. Lett.} {\bf 90} (2003) 021802.

\bibitem{Chau:1984llc}
  Ling-Lie Chau and Wai-Yee Keung,
  Comments on the Parametrization of the Kobayashi-Maskawa Matrix,
  {\it Phys. Rev. Lett.} {\bf 53} (1984) 1802.

\bibitem{Aharmin:2008ba}
  B. Aharmin {\it et al.},
  Electron energy spectra, fluxes, and day-night asymmetries of $^8$B solar neutrinos from measurements with NaCl dissolved in the heavy-water detector at the Sudbury Neutrino Observatory,
  {\it Phys. Rev. C} {\bf 72} (2005) 055502.

\bibitem{Ashie:2004ya}
  Y. Ashie {\it et al.},
  Evidence for an Oscillatory Signature in Atmospheric Neutrino Oscillations,
  {\it Phys. Rev. Lett.} {\bf 93} (2004) 101801.

\bibitem{Apollonio:1999ma}
  M. Apollonio {\it et al.},
  Limits on neutrino oscillations from the CHOOZ experiment,
  {\it Phys. Lett. B} {\bf 466} (1999) 415.

\bibitem{Kraus:2005ck}
  C. Kraus {\it et al.},
  Final Results from phase II of the Mainz Neutrino Mass Search in Tritium $\beta$ Decay,
  {\it Eur. Phys. J. C} {\bf 40} (2005) 447.

\bibitem{Lobashev:1999vml}
  V.~M. Lobashev {\it et al.},
  Direct search for mass of neutrino and anomaly in the tritium beta-spectrum,
  {\it Phys. Lett.} {\bf 460} (1999) 227.

\bibitem{Klapdor-Kleingrothaus:2001kk}
  H. Klapdor-Kleingrothaus {\it et al.},
  Latest results from the HEIDELBERG-MOSCOW double beta decay experiment,
  {\it Eur. Phys. J.} {\bf 12} (2001) 147.

\bibitem{Elgaroy:2003oe} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  O. Elgaroy and O. Lahov,
  {\it J. Cosmol. Astropart. Phys} {\bf 04} (2003) 004.

\bibitem{King:2008sk}
  S. King,
  Measurement of the Double Beta Decay Half-Life of $^{100}$Mo to the $0_1^+$ Excited State, and $^{48}$Ca to the Ground State in the NEMO 3 Experiment,
  PhD Thesis, University College London, 2008.

\bibitem{Gouvea:2006ag}
  A. Gouvea,
  On Determining the Neutrino Mass,
  FNAL Theory Seminar, March 30, 2006.

\bibitem{Curran:1949sc}
  S.~C. Curran, J. Angus, and A.~L. Cockcroft,
  The Beta-Spectrum of Tritium,
  {\it Phys. Rev.} {\bf 76} (1949) 853.

\bibitem{Lobashev:2003vl}
  V.~M. Lobashev,
  The search for the neutrino mass by direct method in the tritium beta-decay and perspectives of study it in the project KATRIN,
  {\it Nucl. Phys. A} {\bf 719} (2003) 153.

\bibitem{Osipowicz:2001ao}
  A. Osipowicz {\it et al.},
  KATRIN: A next generation tritium beta decay experiment with sub-eV sensitivity for the electron neutrino mass,
  {\it Preprint} arXiv:hep-ex/0109033.

\bibitem{Doi:1988md}
  M. Doi, T. Kotani, E. Takasurgi,
  Approximations for double-beta-decay formulas,
  {\it Phys. Rev. C} {\bf 37} (1988) 2104.

\bibitem{Simkovic:1999fs}
  F. Simkovic {\it et al.},
  Additional nucleon current contribution to neutrinoless double $\beta$ decay,
  {\it Phys. Rev. C} {\bf 60} (1999) 055502.

\bibitem{Zuber:2004kz}
  K. Zuber,
  Neutrino Physics,
  {\it Institute of Physics}, 2004.

\bibitem{Ogawa:2003io}
  I. Ogawa {\it et al.},
  Search for neutrino-less double beta decay of $^{48}$Ca by CaF$_2$ scintillator,
  {\it Nucl. Phys. A} {\bf 730} (2004) 215.

\bibitem{Barabash:20006ab}
  A.~S. Barabash {\it et al.},
  NEMO-3 double beta decay experiment: lastest results,
  {\it Preprint} arXiv:hep-ex/0610025.

\bibitem{Danevich:2003fd}
  F.~A. Danevich {\it et al.},
  Search for 2$\beta$ decay of cadmium and tungsten isotopes: Final results of the Solotvina experiment,
  {\it Phys. Rev. C} {\bf 68} (2003) 035501.

\bibitem{Bernatowicz:1993tb}
  T. Bernatowicz {\it et al.},
  Precise determination of relative and absolute $\beta\beta$-decay rates of $^{128}$Te and $^{130}$Te,
  {\it Phys. Rev. C} {\bf 47} (1993) 806.

\bibitem{Arniboldi:2005ca}
  C. Arniboldi {\it et al.},
  Nuclear Quantum Optics with X-Ray Laser Pulses,
  {\it Phys. Rev. Lett.} {\bf 96} (2005) 142501.

\bibitem{Barabash:2005ab}
  A.~S. Barabash {\it et al.},
  Investigation of double-beta-decay processes at the NEMO-3 tracking detector,
  {\it Phys. At. Nucl.} {\bf 68} (2005) 414.

\bibitem{Klapdor:2006hvk}
  H.~V. Klapdor-Kleingrothaus, I.~V. Krivosheina, I.~V. Titkova,
  Particle and nuclear physics parameters-how do they affect the tracks of double beta events in a germanium detector, and their separation from gamma events,
  {\it Physics Letters B} {\bf 632} (2006) 623.

\bibitem{Menendez:2009jm}
  J. Men\'endez,
  Double Beta Decay with Shell Model,
  ILIAS 6th Annual meeting, Dresden, 16-19 February 2009.

\bibitem{Caurier:2008ec}
  E. Caurier, J. Men\'endez, F. Nowacki and A. Poves,
  Influence of Pairing on the Nuclear Matrix Elements of the Neutrinoless $\beta\beta$ Decays,
  {\it Phys. Rev. Lett.} {\bf 100} (2008) 052503.

\bibitem{Simkovic:2008fs}
  F. Simkovic, A. Faessler, V. Rodin, P. Vogel and J. Engel,
  Anatomy of the $0\nu\beta\beta$ nuclear matrix elements,
  {\it Phys. Rev. C} {\bf 77} (2008) 045503,
  {\it Preprint} arXiv:nucl-th/07102055.

\bibitem{Schieffer:2008js}
  J.~P. Schieffer {\it et al},
  Nuclear Structure Relevant to Neutrinoless Double  Decay: $^{76}$Ge and $^{76}$Se,
  {\it Phys. Rev. Lett.} {\bf 100} (2008), 112501.

\bibitem{Kay:2009s}
  B.~P. Kay {\it et al},
  Nuclear structure relevant to neutrinoless double decay: The valence protons in $^{76}$Ge and $^{76}$Se,
  {\it Phys. Rev. C} {\bf 79} (2009), 021301 (R).

\bibitem{Suhonen:2008s}
  J. Suhonen and O. Civitarese,
  Effects of orbital occupancies on the neutrinoless $\beta\beta$ matrix element of $^{76}$Ge,
  {\it Phys. Lett. B} {\bf 668} (2008) 277.

\bibitem{Elliot:2003se}
  S.~R. Elliot and P. Vogel,
  {\it Ann. Rev. Nucl. Part. Sci.} {\bf 52} (2003) 115.

\bibitem{Avignone:2008cs}
  F.~T.~Avignone, S. Elliott and J. Engel,
  Double beta decay, Majorana neutrinos and neutrino mass,
  {\it Rev. Modern. Phys.} {\bf 80} (2008) 481.

\bibitem{Luzon:2006gl}
  G. Luz\'on {\it et al},
  Characterization of the Canfranc Underground Laboratory: Status and future plans,
  Proceedings of the 6th International Workshop on The Identification of Dark Matter, World Scientific, pp. 514-519.

\bibitem{Pandola:2007lp}
  L. Pandola {\it et al.},
  Monte Carlo evaluation of the muon-induced background in the GERDA double beta decay experiment,
  {\it Nucl. Instrum. Meth. A} {\bf 570} (2007) 149.

\bibitem{Gomez:2009hg}
  H. G\'omez,
  Estudio de la sensibilidad de un experimento de desintegraci\'on doble beta con detectores de Ge de nueva generaci\'on,
  PhD thesis, University of Zaragoza, 2009.

\bibitem{Aalseth:1999ca}
  C.~E. Aalseth {\it et al.},
  Neutrinoless double beta decay of $^{76}$Ge: first results from the International Germanium EXperiment (IGEX) with six isotopically enriched detectors,
  {\it Phys. Rev. C}  {\bf 59} (1999) 2108.

\bibitem{Gonzalez:2003dg}
  D. Gonz\'alez {\it et al.},
  Pulse-shape discrimination in the IGEX experiment,
  {\it Nucl. Instrum. Meth.} {\bf 515} (2003) 634.

\bibitem{Gunther:1997mg}
  M. Gunther {\it et al.},
  Heidelberg-Moscow $\beta\beta$ experiment with $^{76}$Ge: full setup with five detectors,
  {\it Phys. Rev. D}  {\bf 55} (1997) 54.

\bibitem{KK:2002kk}
  H. Klapdor-Kleingrothaus {\it et al.},
  Reply to a Comment of article ``Evidence for Neutrinoless Double Beta Decay''
  {\it Preprint} arXiv:hep-ph/0205228.

\bibitem{KK:2003akk}
  H. Klapdor-Kleingrothaus {\it et al.},
  Background analysis around $Q_{\beta\beta}$ for $^{76}$Ge double beta decay experiments, and statistics at low count rates,
  {\it Nucl. Instrum. Meth. A} {\bf 510} (2003) 281.

\bibitem{KK:2003bkk}
  H. Klapdor-Kleingrothaus {\it et al.},
  Measurement of the $^{214}$Bi spectrum in the energy region around the Q-value of $^{76}$Ge neutrinoless double-beta decay,
  {\it Nucl. Instrum. Meth. A} {\bf 511} (2003) 335.

\bibitem{KK:2004kk}
  H. Klapdor-Kleingrothaus {\it et al.},
  Support of evidence for neutrinoless double beta decay,
  {\it Phys. Lett. B} {\bf 578} (2004) 54.

\bibitem{Zdesenko:2002yz}
  Y. Zdesenko {\it et al.},
  Has neutrinoless double $\beta$ decay of $^{76}$Ge been really observed?,
  {\it Phys. Lett. B} {\bf 546} (2002) 206.

\bibitem{Feruglio:2002ff}
  F. Feruglio {\it et al.},
  Neutrino oscillations and signals in $\beta$ and $0\nu2\beta$ experiments,
  {\it Nucl. Phys. B} {\bf 637} (2002) 345.

\bibitem{Giulani:2005ag}
  A. Giuliani {\it et al.},
  Current double beta decay experiments,
  {\it Nucl. Phys. B (Proc. Suppl.)} {\bf 138} (2005) 267.

\bibitem{Arniboldi:2008ca}
  C. Arniboldi {\it et al.},
  Results from a search for the $0\nu\beta\beta$-decay of $^{130}$Te,
  {\it Phys. Rev. C.} {\bf 78} (2008) 035502.

\bibitem{Arniboldi:2003ca}
  C. Arniboldi {\it et al.},
  A calorimetric search on double beta decay of $^{130}$Te,
  {\it Phys. Lett. B} {\bf 557} (2003) 167.

\bibitem{Arnold:2005ara}
  R. Arnold {\it et al.},
  Technical design and performance of the NEMO3 detector,
  {\it Nucl. Instrum. Meth. A} {\bf 536} (2005) 79.

\bibitem{Barabash:2008ab}
  A.~S. Barabash {\it et al},
  Double beta decay: present status,
  {\it Preprint} arXiv:hep-ex/08072948.

\bibitem{Arnold:2004ra}
  R. Arnold {\it et al.},
  Study of $2\beta$-decay of Mo-100 and Se-82 using the NEMO3 detector,
  {\it JETP Lett.} {\bf 80} (2004) 429.

\bibitem{Barabash:2006ab}
  A.~S. Barabash {\it et al.},
  NEMO3 and SuperNEMO double beta decay experiments,
  {\it J. Phys. Conf. Ser.} {\bf 39} (2006) 347.

\bibitem{Vuilleumier:1993jcv}
  J.C. Vuilleumier {\it et al.},
  Search for neutrinoless double-$\beta$ decay in $^{136}$Xe with a time projection chamber,
  {\it Phys. Rev. D} {\bf 48} (1993) 1009.

\bibitem{Maj:2003}
  The Majorana Collaboration,
  White Paper on the Majorana Zero- Neutrino Double-Beta Decay Experiment,
  {\it Preprint} arXiv:nucl-ex/0311013.

\bibitem{Elliot:2006se}
  S. Elliot {\it et al.},
  The Majorana project,
  {\it J. Phys. Conf. Ser.} {\bf 39} (2006) 341.

\bibitem{Abt:2004ia}
  I. Abt {\it et al.},
  GERDA Letter of Intent, A new $^{76}$Ge Double Beta Decay Experiment at LNGS,
  {\it Preprint} arXiv:hep-ex/0404039.

\bibitem{Majorovits:2008bm}
  B. Majorovits,
  The GERDA neutrinoless-double-beta decay experiment,
  {\it Proceedings of Science, IDM 2008} (2008) 69.

\bibitem{Arnaboldi:2004ca}
  C. Arnaboldi {\it et al.},
  CUORE: a cryogenic underground observatory for rare events,
  {\it Nucl. Instrum. Meth. A} {\bf 518} (2004) 775.

\bibitem{Danilov:2000md}
  M. Danilov {\it et al.},
  Detection of very small neutrino masses in double-beta decay using laser tagging 
  {\it Phys. Lett. B} {\bf 480} (2000) 12.

\bibitem{Leo:1994wl}
  W.~R. Leo,
  Techniques for Nuclear and Particle Physics Experiments,
  Springer-Verlag Berlin Heidelberg, 1994.

\bibitem{Blum:1994wb}
  W. Blum and L. Rolandi,
  Particle Detection with Drift Chambers,
  Springer-Verlag Berlin Heidelberg, 1993.

\bibitem{Berger:2009mjb}
  M.~J. Berger {\it et al.},
  XCOM: Photon Cross Sections Database,
  National Institute of Standarts and Technology (NIST).

\bibitem{Groom:dg}
  D.~E. Groom, N.V. Mokhov and S.I. Striganov,
  Muon stopping power and range tables 10 MeV - 100 TeV.

\bibitem{Wikipedia}
  Wikipedia encyclopedy,
  Helmut Paul (own work),
  9th May 2006.

\bibitem{Christophorou:1971lc}
  L.~G. Christophorou,
  Atomic and Molecular Radiation Physics,
  Wiley, London 1971.

\bibitem{Chefdeville:2009mc}
  M. Chefdeville,
  Development of Micromegas-like gaseous detectors using a pixel readout chip as collecting anode,
  PhD Thesis, University of Amsterdam, 2009.

\bibitem{Biagi:1988sb}
  S.~F. Biagi,
  Accurate solution of the Boltzmann transport equation,
  {\it Nucl. Instrum. Meth. A} {\bf 273} (1988) 533.

\bibitem{Stacey:2005bs}
  B. Stacey,
  Relation of Electron Scattering Cross-Sections to Drift Measurements in Noble Gases,
  Bachelor thesis, MIT, June 2005.

\bibitem{Ramsauer:1921cr}
  C. Ramsauer,
  Uber den Wirkungsquerschnitt der Gasmolekule gegenuber langsame Elektronen,
  {\it Ann. Phys.} {\bf 66} (1921) 546.

\bibitem{Christophorou:1980lc}
  L.~G. Christophorou, D.~V. Maxey, D.~L. McCorkle and J.~G. Carter,
  Xe-containing fast mixtures for gas-filled detectors,
  {\it Nucl. Instrum. Meth.} {\bf 171} (1980) 491.

\bibitem{Biagi:1999sb}
  S.~F. Biagi,
  Montecarlo simulation of electron drift and diffusion in counting gases under the influence of electric and magnetic fields,
  {\it Nucl. Instrum. Meth.} {\bf 421} (1999) 234
  Programme and cross sections available in http://www.cern.ch/magboltz.

\bibitem{Sauli:1984fs}
  A. Peisert and F. Sauli,
  Drift and Diffusion of electrons in gases: A compilation,
  CERN 84-08, Experimental Physics Division, 1984.

\bibitem{Jean-Marie:1979bjm}
  B. Jean-Marie, V. Lepeltier and D. L'Hote,
  Systematic measurement of electron drift velocity and study of some properties of four gas mixtures: A-CH$_4$, A-C$_2$H$_4$, A-C$_2$H$_6$, A-C$_3$H$_8$,
  {\it Nucl. Instrum. Meth.} {\bf 152} (1979) 541.

\bibitem{Andronic:2004aa}
  A. Andronic et al.,
  Drift velocity and gain in argon- and xenon-based mixtures,
  {\it Nucl. Instrum. Meth. A} {\bf 523} (2004) 302.

\bibitem{Berghofer:2004tb}
  Th. Berghofer, J. Blumer, J.~R. Horandel,
  A measurement of drift velocities of electrons in xenon-methane mixtures,
  {\it Nucl. Instrum. Meth. A} {\bf 525} (2004) 544.

\bibitem{McCorkle:1981dm}
  D.~L. McCorkle, L.~G. Christophorou and S.~R. Hunter,
  Electron attachment rate constants and cross-sections for halocarbons,
  Proc. Second International Swarm Seminar, Oak Ridge, USA, 1981,
  Pergamon, New York, 1981.

\bibitem{Shimamori:1984hs}
  H. Shimamori and H. Hotta,
  Mechanism of thermal electron attachment to O$_2$: Isotope effect studies with $^{18}$O$_2$ in rare gases and some hydrocarbons,
  {\it J. Chem. Phys.} {\bf 81} (1984) 1271.

\bibitem{Huk:1988mh}
  M. Huk, P. Igo-kemenes and A. Wagner,
  Electron attachment to oxygen, water and methanol in various drift chamber gas mixtures,
  {\it Nucl. Instrum. Meth. A} {\bf 267} (1988) 107.

\bibitem{Hunter:1989sh}
  S.~R. Hunter, J.~G. Carter and L.~G. Christophorou,
  Low energy electron attachment to SF$_6$ in N$_2$, Ar and Xe buffer gases,
  {\it J. Chem. Phys.} {\bf 90} (1989) 4879.

\bibitem{Andronic:2003aa}
  A. Andronic {\it et al.},
  Pulse height measurements and electron attachment in drift chambers operated with Xe,$CO_2$ mixtures,
  {\it Preprint} arXiv:physics/0303059v1.

\bibitem{Kuffel:1959ek}
  E. Kuffel,
  Condensation Nuclei produced by the Ultra-violet Irradiation of Humid Air or Humid Argon,
  {\it Proc. Phys. Soc.} {\bf 74} (1959) 297.

\bibitem{Rose:1941mr}
  M.~E. Rose and S.~A. Korff,
  An Investigation of the Properties of Proportional Counters. I,
  {\it Phys. Rev.} {\bf 59} (1941) 850.

\bibitem{Sauli:1998fs}
  F. Sauli,
  Gas detectors: Recent developments and future perspectives,
  {\it Nucl. Instrum. Meth. A} {\bf 419} (1988) 189.

\bibitem{Sauli:1999fs}
  F. Sauli and A. Sharma,
  Micropattern Gaseous Detectors,
  {\it Annu. Rev. Nucl. Part. Sci} {\bf 49} (1999) 341.

\bibitem{Geiger:1908hg}
  H. Geiger, E. Rutherford,
  An Electrical Method of Counting the Number of $\alpha$-Particles from Radio-Active Substances,
  {\it Proc. Royal Soc. A} {\bf 81} (1908) 141.

\bibitem{Geiger:1928hg} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  H. Geiger, W. Muller,
  {\it Phys. Zeits.} {\bf 29} (1928) 839.

\bibitem{Charpak:1968}
  G. Charpak {\it et al.},
  The use of multiwire proportional counters to select and localize charged particles,
  {\it Nucl. Instrum. Meth.} {\bf 62} (1968) 262.

\bibitem{Nygren:1978dn}
  D.~R. Nygren and J.~N. Marx,
  The Time Projection Chamber,
  {\it Physics Today} {\bf 31} (1978), 46.

\bibitem{Oed:1988ao}
  A. Oed,
  Position-sensitive detector with microstrip anode for electron multiplication with gases,
  {\it Nucl. Instrum. Meth. A} {\bf 263} (1988) 351.

\bibitem{Charpak:1992gc}
  G. Charpak,
  Nobel Lecture, 1992.

\bibitem{Kleinknecht:1998jk}
  K. Kleinknecht,
  Detectors for particle ratidation,
  2nd edition, Cambridge University Press, Cambridge (1998).

\bibitem{Bouclier:1993rb}
  R. Bouclier {\it et al.},
  Performance of gas microstrip chambers on glass substrata with electronic conductivity,
  {\it Nucl. Instrum. Meth. A} {\bf 332} (1993) 100.

\bibitem{Angelini:1990fa}
  F. Angelini {\it et al.},
  Test-beam study of the performance of the microstrip gas avalanche chamber,
  {\it IEEE Trans. Nucl. Sci.} {\bf 37} (1990) 112.

\bibitem{Sauli:2001fs}
  F. Sauli,
  Gas detectors: achievements and trends,
  {\it Nucl. Instrum. Meth. A} {\bf 461} (2001) 47.

\bibitem{Bohm:1995jb}
  J. Bohm,
  High rate operation and lifetime studies with micro-strip gas chambers,
  {\it Nucl. Instrum. Meth. A} {\bf 360} (1995) 34.

\bibitem{Barr:1998ab}
  A. Barr,
  Construction, test and operation in a high intensity beam of a small system of micro-strip gas chambers,
  {\it Nucl. Instrum. Meth. A} {\bf 403} (1998) 31.

\bibitem{Sauli:1997fs}
  F. Sauli,
  GEM: A new concept for electron amplification in gas detectors,
  {\it Nucl. Instrum. Meth. A} {\bf 386} (1997) 531.

\bibitem{Zeuner:2000tz}
  T. Zeuner,
  The MSGC-GEM Inner Tracker for HERA-B,
  {\it Nucl. Instrum. Meth. A} {\bf 446} (2000) 324.

\bibitem{Ketzer:2004bk}
  B. Ketzer {\it et al.},
  Trends and highlights of VCI 2004,
  {\it Nucl. Instrum. Meth. A} {\bf 535} (2004) 79.

\bibitem{Raspino:2007dr}
  D. Raspino {\it et al.},
  Status of triple GEM muon chambers for the LHCb experiment,
  {\it Nucl. Instrum. Meth. A} {\bf 581} (2007) 283.

\bibitem{Ruggiero:2005gr}
  G. Ruggiero,
  The TOTEM Detectors,
  {\it Proc. of the XI$^{th}$ International Conference of Elastic and Diffractive Scattering Towards the High Energy Frontiers}, Blois, France (2005).

\bibitem{Tserruya:2004it}
  I. Tserruya,
  Development of a triple GEM UV-photon detector operated in pure CF4 for the PHENIX experiment,
  {\it Nucl. Instrum. Meth. A} {\bf 523} (2004) 345.

\bibitem{Peyaud:2004by}
  B. Peyaud {\it et al},
  KABES: a novel beam spectrometer for NA48,
  {\it Nucl. Instrum. Meth. A} {\bf 535} (2004) 247.

\bibitem{Aune:2007sa}
  S. Aune {\it et al.},
  Performance of the micromegas detector in the CAST experiment,
  {\it Nucl. Instrum. Meth.  A} {\bf 573} (2007) 38.

\bibitem{FerrerRibas:2007efr}
  E. Ferrer-Ribas {\it et al},
  A new Micromegas line for the CAST experiment,
  {\it Nucl. Instrum. Meth. A} {\bf 581} (2007) 217.

\bibitem{Kunne:2005fk}
  F. Kunne {\it et al},
  The $40 \times 40$ cm$^2$ gaseous microstrip detector Micromegas for the high-luminosity COMPASS experiment at CERN,
  {\it Nucl. Instrum. Meth. A} {\bf 536} (2005) 61.

\bibitem{Kudenko:2009yk}
  Y. Kudenko {\it et al},
  The near neutrino detector for the T2K experiment,
  {\it Nucl. Instrum. Meth. A} {\bf 598} (2009) 1.

\bibitem{Giomataris:1998yg} 
  Y. Giomataris,
  Development and prospects of the new gaseous detector Micromegas,
  {\it Nucl. Instrum. Meth. A} {\bf 419} (1998) 239.

\bibitem{Barouch:1999gb}
  G. Barouch {\it et al.},
  Development and prospects of a fast gaseous detector Micromegas,
  {\it Nucl. Instrum. Meth. A} {\bf 423} (1999) 32.

\bibitem{Vavra:1993jv}
  J. Va'vra {\it et al.},
  Measurement of electron drift parameters for helium and CF$_4$-based gases,
  {\it Nucl. Instrum. Meth. A} {\bf 324} (1993) 113.
  
\bibitem{Derre:2000jd}
  J. Derr\'e {\it et al.},
  Fast signals and single electron detection with a MICROMEGAS photodetector,
  {\it Nucl. Instrum. Meth. A} {\bf 449} (2000) 314.

\bibitem{Mols:2009jpm}
  J.P. Mols and E. Ferrer-Ribas,
  photographs at the microscope reproduced with permission.

\bibitem{Delbart:2001ad}
  A. Delbart {\it et al.},
  New developments of Micromegas detector,
  {\it Nucl. Instrum. Meth. A} {\bf 461} (2001) 84.

\bibitem{Jeanneret:2003pj}
  P. Jeanneret {\it et al.},
  Performance of a new Micromegas detector, with woven wire mesh,in $CF_4$,
  {\it Nucl. Instrum. Meth. A} {\bf 500} (2003) 133.

\bibitem{Ounalli:2008ue}
  L. Ounalli, J.~L. Vuilleumier, D. Schenker and J.~M. Vuilleumier,
  New gas mixtures suitable for rare event detection using a Micromegas TPC detector,
  {\it JINST} {\bf 4} (2009) P01001,
  {\it Preprint} arXiv:hep-ex/0810.0445.

\bibitem{Derre:2001jd}
  J. Derr\'e {\it et al.},
  Spatial resolution in Micromegas detector,
  {\it Nucl. Instrum. Meth. A} {\bf 459} (2001) 523.

\bibitem{Derre:1998jd}
  J. Derr\'e {\it et al.},
  First beam test results with Micromegas, a high-rate, high-resolution detector,
  {\it Nucl. Instrum. Meth. A} {\bf 412} (1998) 47.

\bibitem{Delbart:2002ad}
  A. Delbart {\it et al.},
  Performance of MICROMEGAS with preamplification at high intensity hadron beams,
  {\it Nucl. Instrum. Meth. A} {\bf 478} (2002) 205.

\bibitem{Giomataris:2006yg}
  I. Giomataris {\it et al.},
  Micromegas in a bulk,
  {\it Nucl. Instrum. Meth. A} {\bf 560} (2006) 405,
  {\it Preprint} arXiv:physics/0501003.

\bibitem{Papaevangelou:2008tp}
  T. Papaevangelou,
  Talk Given at the Fourth Symposium on Large TPCs for Low Energy Rare Event Detection,
  Paris, December 18-19, 2008 $<$http://www-tpc-paris.cea.fr$>$.

\bibitem{Messer:2009me}
  Messer Industriegase GmbH,
  http://www.messergroup.com/.

\bibitem{Knoll:2000gk}
  Glenn F. Knoll,
  Radiation Detection and Measurement.
  John Wiley and Sons, 3rd edition, 2000.



\bibitem{Bolotnikov:1999ab}
  A. Bolotnikov and B. Ramsey,
  Studies of light and charge produced by alpha-particles in high-pressure xenon,
  {\it Nucl. Instrum. Meth. A} {\bf 428} (1999) 391.

\bibitem{Meinschad:2005tm}
  T. Meinschad, L. Ropelewski and F. Sauli,
  Detection ofprimary and field-enhanced scintillation in xenon with a CsI-coated GEM detector,
  {\it Nucl. Instrum. Meth. A} {\bf 547} (2005) 342.

\bibitem{Braem:2009ab}
  CsI deposit made by Andr\'e Braem (CERN-PH).

\bibitem{Tomas:2010at}
  A. Tom\'as,
  PhD. Thesis in preparation, University of Zaragoza, 2010.

\bibitem{Saes:2009sa}
  SAES Getters S.p.A.,
  http://www.saesgetters.com/.
  
\bibitem{Curioni:2009ac}
  A. Curioni {\it et al},
  A regenerable filter for liquid argon purification,
  {\it Nucl. Instrum. Meth. A} {\bf 605} (2009) 306.

 \bibitem{Pokratenko:2000op}
  O.~A. Pokratenko {\it et al.},
  Event generator DECAY4 for simulation of double beta processes and decays of radiactive nuclei,
  {\it Phys. At. Nucl.}, {\bf 63} (2000) 1282-1287.

\bibitem{Agostinelli:2003sa}
  S. Agostinelli {\it et al.},
  GEANT4-a simulation tookit,
  {\it Nucl. Instrum. Meth. A} {\bf 506} (2003) 250-303.

\bibitem{Allison:2006ja}
  J. Allison {\it et al.},
  GEANT4 developments and applications,
  {\it IEEE Transactions on Nuclear Science} {\bf 53} (2006) 270.

\bibitem{Geant4:2005ge}
  GEANT4 Collaboration,
  Physics Reference Manual,
  http://geant4.cern.ch (2005).

\bibitem{ROOT:2000}
  ROOT,
  a framework for data processing,
  http://root.cern.ch.

\bibitem{SRIM:2008}
  SRIM,
  the Stopping and Range of Ions in Matter,
  http://www.srim.org.

\bibitem{Luzon:2009gl}
  G. Luz\'on,
  private communication.

\bibitem{ToIDD}
  Table of Isotopes Decay Data,
  http://nucleardata.nuclear.lu.se/nucleardata/toi.

\bibitem{Castell:2009jc}
  J. Castell,
  private communication.

 \bibitem{ILIAS:2009rp}
  ILIAS database on radiopurity of materials,
  http://radiopurity.in2p3.fr.

 \bibitem{Maneschg:2008ma}
  W. Maneschg {\it et al.},
  Measurements of extremely low radioactivity levels in stainless steel for GERDA,
  {\it Nucl. Instrum. Meth. A} {\bf 593} (2008) 448.

 \bibitem{Aprile:2008ap}
  E. Aprile {\it et al.},
  The search for dark matter with the XENON experiment,
  Talk Given at the Fourth Symposium on Large TPCs for Low Energy Rare Event Detection,
  Paris, December 18-19, 2008 $<$http://www-tpc-paris.cea.fr$>$.

 \bibitem{Heusser:2004he}
  G. Heusser,
  Low level counting from meteorites to neutrinos,
  {\it Proc. Low Radioactive Techniques} 2004 p. 29.

\bibitem{Olaverri:2005ao}
  A.~G. Olaverri,
  Teor\'ia de grafos y combinatoria,
  Subject notes, University of Zaragoza.

 \bibitem{Wong:2009wg}
  H.~T. Wong, D.~A. Imel, V. J\"orgens, M. Treichel and J.~C. Vuilleumier,
  Event identification with a time projection chamber in a double beta decay experiment on $^{136}$Xe,
  {\it Nucl. Instrum. Meth. A} {\bf 329} (1993) 163.

\bibitem{Gomez:2009hg2}
  H.~Gomez {\it et al},
  article in preparation.

\end{thebibliography}

